Not Just Duolingo: Supporting Immigrant Language Preservation Through Family-Based Play

For immigrants, language preservation is crucial to maintain their identity, but the process of immigration can put a strain on a community's ability to do so. We interviewed eight Nepali immigrants to understand barriers to language preservation across sociopolitical contexts in Nepal and immigrant life in the United States. Participants described strong motivation but limited institutional support, time and resource constraints, and English-dominant environments that widen parent-child language gaps. They envisioned technology that supports interactive, family centered learning. In response, we are developing an audio-first, point-and-click language learning game based on the theory of comprehensible input, designed for parent-child co-playing. An early evaluation with four design experts reveals promising gameplay, and the need to simplify symbol-heavy UI. We conclude with implications for designing language technologies that support preservation through relations while acknowledging the limits of design.

==> contents/long_paper/design-intervention.tex <==
\subsection{Design Intervention}
\label{design-intervention}

% \subsection{Design Process} 
% %%% Question to answer in this section while you talk about the game: why did you design the game the way you did? When you are answering this, connect it to the findings in Section 4. 
% %% Basically, justify your design decisions based on the empirical data. 

% % Based on the technological interventions described by the participants, we are developing a language learning game intended to foster parent-child connection.
% We utilized the double diamond model \cite{kochanowska_double_2022} to ideate on design solutions.
% First, we identified common issues present in our themes (e.g., "lack of linguistic pride", "no school curriculum", etc.), then narrowed down our scope, focusing on "a lack of learning resources" and "emotional barriers between parents and children".
% This led to the second half of the double diamond model, discussing potential design solutions. 
% We decided on a game-based solution to encourage both language learning and parent-child bonding to address participant desires for interactivity and parent inclusion.

\subsubsection{Game Design}
\label{game-design}
%% We repeat some parts to justify why we designed our game the way we did
Our design is motivated by the participants' desires for interactivity that go beyond traditional language learning games (Section \ref{technology-interventions-for-language-preservation}).
As such, our game is audio-only, based on the theory of comprehensible input \cite{tarekhamza2016, rodrigo2004}, to create an engaging language learning experience.
To reduce the entry barrier (Section \ref{motivations-for-language-learning}), we use point-and-click mechanics (Figure \ref{fig:game}). %% because participants said this or that. 
And lastly, we envision the child playing the game directly, with the parent serving as a mentor to scaffold learning while bonding with their child (Sections \ref{issues-facing-Indigenous-language-learning} and \ref{technology-interventions-for-language-preservation}).
% The child has control over the physical activity, and the parent can provide their verbal language knowledge (Section \ref{technology-interventions-for-language-preservation}).

We develop with the Godot Engine \cite{linietsky_godot_nodate}, and assets are drawn Inkscape, or obtained through Flaticon\footnote{\url{https://www.flaticon.com/}}, free for commercial use (with attribution).
% \footnote{All icons are attributed in the game files, which will be public upon the project's completion.}.
% Finally, audio recordings were split between an Audicity-based pipeline and ad hoc recording for Mandarin Chinese.
% We plan to standardize this pipeline going forward for smoother translation and audio inclusion.
Our prototype has translations for Spanish and Mandarin Chinese, but
future work will involve Nepali Indigenous languages spoken by native speakers.
The game play consists of story scenes where the player must complete a task.
Since grocery shopping is a common experience, we use this setting to prioritize game play prior to incorporating cultural elements.
Upon starting the game, players listen to a recording in the target language stating the task.
These recordings are simple, indicative sentences (e.g., ``you put an apple in the shopping cart'').
We avoid using commands or complex sentences to focus on beginner learners \cite{}.

Interactable objects will glow when the mouse hovers.
Clicking an object shows a radial menu with its available actions. 
Actions will always include listening to the object's name.
Other possible actions include eating or carrying the object depending on the individual item.
When the player completes an action, the involved icons are shown in the "action panel". Completing actions will always form a valid sentence.
Players can then listen to the created sentence, submit their answer, or clear the action (Figure \ref{fig:game}).
If the player is wrong, an "incorrect answer" jingle plays, and the display is cleared.
If the player is correct, a "correct answer" jingle plays, and the game transitions to the next scene.

% We try to have each scene in the story make sense, building off previous steps taken in the story.
% However, our system is extremely flexible, and future work plans to look at altering the stories for more advanced language learners. 
% For example, we can easily change the complexity of the audio for the task, making audios be less direct (e.g., ``You want to make a cake, get what you need to make a cake in the cart'') or make the task more unusual (e.g., having the player eat the apple they just bought).

\subsubsection{Early Prototype Evaluation}
\label{early-prototype-evaluation}

We ran play tests with three HCI researchers and a game designer to identify major issues. This allows us to refine the game before conducting parent-child studies.
Each play tester was briefed of the game's intended audience (immigrant parents and their children), as well as a short introduction to the game's mechanics (listen to audio, click on objects to interact with them, etc.).
Play testers were encouraged to select a language they did not speak. Three designers selected Spanish and one selected Chinese.
We avoided disclosing action symbol meaning to see if our UI was intuitive.

After finishing, we deployed the EOTA method \cite{hammer2018eota} to elicit feedback from the participants.
We noted participant game play and highlighted points of friction.
Each session took thirty minutes to an hour to complete.
Lastly, we conducted a round of thematic analysis with the feedback and our field notes.


\subsubsection{Initial Feedback}
\label{initial-feedback}

Initial feedback has been positive, and the designers enjoyed playing the game.
All designers successfully utilized the object audio to decipher the task audio quickly.
Two designers stated that later levels were too easy due to recognizable pattern repetition. %This could be due to lack of task variety in our prototype.
Some reported confusion with the radial menus. One designer was confused about the "eat" symbol (utensils), and another on how to pick up objects.
Critically, all designers found the action panel to be unclear, with most not understanding how to navigate it due to the heavy use of symbols.
% We believe this is a side affect of action symbol confusion, and future prototypes will work to address these action symbol and action panel issues.
% We will also consider these changes going forward as we want our game to be intuitive to our target demographic, who might have differing technological knowledge.

The designers suggested having an object's audio play automatically when clicked, overhauling the action panel by reducing information load, and refining symbols.
Lastly,in reference to our target demographic the designers recommended parent engagement via game participation rather than stictly observing. %% Connect to literature and then talk about why this matters to us and what we are going to do about it. 
% This feedback matches with previous literature on parental participation in gaming activities, which finds that parents engage with games in a wide variety of ways \cite{pais2025}, and is critical to consider if we are to make an engaging experience for both the parent and child.
% Our design was too focused on preventing the parent from overtaking the experience, which---while still a concern \cite{einarsson2022, yu2023}---restricted the possible roles for the parent.
% But now, synthesizing this feedback with the interviews, we plan to experiment with the story aspect of the game, looking at how the parent can participate, and play a more central role in the game. 

==> contents/long_paper/findings-design.tex <==
\section{Findings and Design}
\label{findings-and-design}

% @YY and Alejandro, can you start porting the content from the Google doc to here?

% Remember, the goal is to show why the family-involved game is needed. Justify the design. 

% A thematic analysis on interviews with eight participants provided insights into the current perspectives regarding the preservation of Indigenous languages in Nepal and the United States.
We find that the desire for language preservation arose from personal identity but is challenged by environmental contexts, and that ideations on technological interventions focused on the potential of play and interactivity.
% We elaborate on these findings below.

%\subsection{Political Complications}
% \label{political-complications}

%% MAPPING (TENTATIVE TO CHANGE UNTIL I POST IT IN THE SLACK!!!)
%% P6 -> P1
%% P7 -> P2
%% P8 -> P3
%% P9 -> P4
%% P11 -> P5
%% P20 -> P6
%% P24 -> P7
%% P31 -> P8
% ADD QUOTES FROM P11 (P5) AND P24 (P7)

\subsection{Interview Findings}
\label{interview-findings}


\subsubsection{Issues Facing Indigenous Languages Learning}
\label{issues-facing-Indigenous-language-learning}
In the United States, immigrants are pressured to choose between their culture and assimilation.
As P4 explains, ``Maybe it is identity crisis, or survival mode . . . I cannot use the American mentality in Nepali society and vice-versa.''
P3 had similar thoughts, ``When I tried to apply cultures I learned in Nepal [in the U.S.], I could not assimilate.
Then I became someone who wants to be like Americans, learn their culture.''
P8 mentioned the parental influence, ``[parents] want their children to speak like native English speakers. . . .
Those immigrated parents realize their struggle in a new place because of English.'' This tension to assimilate can thus deter language preservation efforts.

Within the Nepali context, impartial reform to include Indigenous languages in formal education are complicated by the country's linguistic diversity.
As P3 expressed, ``. . . I have my doubts because Nepal, although small, is a diverse country . . .  adding in curriculum might raise questions from people why their language is not being represented.'' 
Since there is no clear and equitable solution to include all Indigenous languages in the formal curriculum, the movement for systematic change currently remains at a standstill. 

Without a formal curriculum, Indigenous languages exist primarily in private spaces and rely on family circles to keep them alive.
% Several participants alluded to a strong relationship between the functionality of a language and the frequency of its usage.
For example, P2 provided their perspective, ``I think Indigenous languages are spoken mainly outside of Kathmandu valley, in rural communities.
Even in those communities, it is spoken within the family, inside that house only.'' 
Similarly, P4 shared, ``the majority of Limbu learned the language by listening, no one has learned it in an academic environment because of the political scenario, scripts, language were not taught.''
P3 supported this, ``I was not taught the language in school either. . . . 
I used to hear grandmothers speak it since when I was a child and I learned the language based on just listening.''
We see that continued use within families becomes vital for Indigenous languages as they are not widely circulated in institutional settings. 

\subsubsection{Motivations for Language Learning}
\label{motivations-for-language-learning}

The responsibilities of daily life can demotivate individuals from pursuing language learning.
%As P24 shared, ``I don’t think I would be convinced if someone tried to put me in a language class at this age.
%The importance and respect that needs to be held for languages fades away...''
P8 shares, ``There could be some people who are serious about language preservation and are actively involved in it; those people might read those books.
However, for other people those books are extra expense and demanding of their time.
So, at the end of the day, it is about the personal commitment of a person.''
Learning an Indigenous language is a costly and a time consuming endeavor requiring individual motivation. 

The desire to connect with family motivates an individual to (re)learn a language.
As P3 states, ``I feel amazing talking to my seniors using my languages but I feel upset as well that I cannot speak it fluently.''
Similarly, P1 shared, ``My grandfather was actively involved in this language preservation.
. . . I would find his notepad where the history of Maithili language . . . were written I learned about the history of the language from there.''
P1's grandfather's preservation efforts served as a spark for P1's language learning, and thus, the desire to connect with family can be a critical source of motivation. 

Likewise, this extends to keeping younger generations connected as well.
For instance, P6 explained, ``The other reason I want them to know Newari is for them to be able to talk to their grandparents.
I don't want them to talk in English while my parents talk in Newari and Nepali.''
P8 further supports this, `` . . . when immigrant parents speak English with their children born in the USA, there is a gap when it comes to expressing the emotion from the parents' end because their comfort language is different from English . . . ''
This gap can create tension and weaken parent-child relationships, further motivating the need for language preservation.

\subsubsection{Technology Interventions for Language Preservation}
\label{technology-interventions-for-language-preservation}

To mediate these concerns, participants suggested the incorporation of modern technology and prioritizing the family to develop new language learning material.
P4 mentions, ``Children also learn from hearing those languages in their surroundings.
If there could be an environment for kids to be in those surroundings, it could be playing games, online games, etc.
Parents should also be involved in it.''
% Thus, we see a desire for an interactive, parent-involved language learning experience.
In addition to this, P6 also suggested making more story-based materials, ``Rather than focusing on writing scripts, maybe we can start sharing the stories out of there . . . ''
% Making more digestible modes of media could allow less interested or external crowds to pay attention and participate.
However, P4 recommends caution, ``I do not think we should build something that’s Duolingo from 2012 but there could be something where people can live and interact, chat with others rather than machines.''
The emphasis on parent-inclusive, interactive, digestible language learning experiences highlights important elements that technological solutions should explore.
% The emotional depth from storytelling can prevent the gaming elements from overshadowing the purpose of language learning. 


==> contents/long_paper/findings.tex <==
\section{Findings}

% @YY and Alejandro, can you start porting the content from the Google doc to here?

% Remember, the goal is to show why the family-involved game is needed. Justify the design. 

Interviews with eight participants provided insight into the current perspectives concerning the preservation of
Indigenous languages in Nepal.
Upon conducting a thematic analysis of the interview transcripts, several overarching themes emerged.
We find that attitudes towards language preservation arose from personal identity and are influenced by social context and the surrounding environment of the individual.
We outline the identified limitations on current language preservation efforts and detail technological interventions suggested by the participants. 

\subsection{Institutional Restriction}

Establishing an impartial reform to include the indigenous language in formal education becomes complicated due to the occupation of various languages in a given region of Nepal. P8 expressed, “To talk about adding in school curriculum, I have my doubts because Nepal, although small, is a diverse country. Thus, adding in curriculum might raise questions from people why their language is not being represented. Deciding which state shall represent which language is also a point of discussion on a political level." Because there is no clear and equitable solution to include all indigenous languages in the formal curriculum, the movement for systematic change currently results in a standstill. 

\subsection{Primary learning Method of Indigenous Languages}

Without a formal curriculum, the presence of indigenous languages exists primarily in private spaces and is dependent on close social circles to pass on and maintain. Several participants alluded to a strong relationship between the functionality of a language and the frequency of usage. For example, P7 provided their perspective, “I think indigenous languages are spoken mainly outside of Kathmandu valley, in rural communities. Even in those communities, it is spoken within the family, inside that house only.” Similarly, P9 shared, “Now, in the case of Limbu, the majority of Limbu learned the language by listening, no one has learned it in an academic environment because of the political scenario, scripts, language were not taught.” P8 supported this, “I was not taught the language in school either. Limbu was like ‘mukh bata jhareko bhasa’. I used to hear grandmothers speak it since when I was a child and I learned the language based on just listening.” Continued encouragement in these social circles becomes especially pertinent for indigenous languages that are not widely circulated in institutionalized settings. 

\subsection{Motivation for Language Learning}

Because the circulation of these languages are reliant on the individual, the responsibilities of daily life demotivates the individual from pursuing language learning. P24 shared, “I don’t think I would be convinced if someone tried to put me in a language class at this age. The importance and respect that needs to be held for languages fades away at my age.” P31 agreed with a similar point, “There could be some people who are serious about language preservation and are actively involved in it; those people might read those books. However, for other people those books are extra expense and demanding of their time. So, at the end of the day, it is about the personal commitment of a person.” Learning an indigenous language is a costly and time consuming endeavor and ultimately requires motivation to pursue. 

The desire to speak with family motivates an individual to learn or relearn a language. The experience of P8 highlighted, “I feel amazing talking to my seniors using my languages but I feel upset as well that I cannot speak it fluently.” P8 felt rewarded by communication with her family and proportionally developed emotional distress when the desired level of fluency was not achieved. In a similar manner, P6 provided the reason their childhood self was inspired by the Maithili language, “My grandfather was actively involved in this language preservation. When I was a child, I would find his notepad where the history of Maithili language, its origin were written. I learned about the history of the language from there.” The exposure to their family’s interest in language learning served as motivation for subsequent language learning in the child. Personal motivation to learn the language stems from a desire to connect with family. 

Likewise, the motivation to then teach the language stems from a desire to keep younger generations connected with family.  For instance, P20 explained, “The other reason I want them to know Newari is for them to be able to talk to their grandparents. I don't want them to talk in English while my parents talk in Newari and Nepali.” a language barrier will be created between family members if younger generations are not taught their family’s respective indigenous language.  P31 claimed, “In my perspective, when immigrant parents speak English with their children born in the USA, there is a gap when it comes to expressing the emotion from the parents' end because their comfort language is different from English and they chose to speak English because of circumstantial reasons.” The language gap between generations continues to expand as globalization and migratory factors place indigenous language learning in the background. 

\subsection{Incorporation of Technology}

To mediate these issues, participants suggested the incorporation of modern technology and family involvement to develop a new interactive space in language learning. P9 described, “Children also learn from hearing those languages in their surroundings. If there could be an environment for kids to be in those surroundings, it could be playing games, online games, etc. Parents should also be involved in it.” The utilization of games attracts and retains attention. In addition to entertainment, P20 suggested, “Rather than focusing on writing scripts, maybe we can start sharing the stories out of there. Sharing the stories, sharing how it is different.” Making more digestible modes of media can allow less interested or external crowds to pay attention and participate. Additionally, P9 described, “I do not think we should build something that’s Duolingo from 2012 but there could be something where people can live and interact, chat with others rather than machines.” The emotional depth from storytelling can prevent the gaming elements from overshadowing the purpose of language learning. 


==> contents/long_paper/related-work.tex <==
\section{Related Work}

% These are suggested subsections. Of course, change it if it helps in structuring the findings. 
Our work sits at the intersection between HCI's work on language preservation and promotion efforts in migrant populations and game design (as well as broader joint media experience research), particularly family-based game design and game design for cultural and language preservation. We provide a brief overview of these fields and our contributions to each.

\subsubsection{Culture and Language Preservation with Migrant Populations}

Within the broader scope of general language preservation and promotion efforts, there exist drastic differences in their scopes, resources and capacity depending on the sociopolitical contexts language communities face \cite{hinton2018a}. %% You need citations here. 
Furthermore, which cultural practices and traditions are emphasized and which are further marginalized are also subject to change due to generational, academic, and multilingual influences \cite{hinton2018a, hornberger2023a, riestenberg2024a}.
Importantly, while academic interventions have provided benefits for language preservation and promotion efforts, the pre-existing conditions that much of academia has been founded in (namely colonialism and the ``publish or perish mindset'') have caused tensions between academic institutions and language communities \cite{riestenberg2024a}.

Previous migrant-focused work in HCI, CSCW and other human-focused computing fields largely focuses on either addressing more direct needs of migrant communities (e.g., \cite{georgiou2023, pei2020, aal2014, he2025, chang2024}) or exploring how the act of migration affects participants (e.g., \cite{brown2012, lei2024, tachtler2020, shi2025}).
The intersection between HCI and cultural preservation efforts, especially how HCI can develop cultural preservation technologies for and with migrant communities, remains an understudied area of research \cite{sabie2022}. 
Existing work in this area has largely focused on cultural preservation through memory, exploring how memories, storytelling and speculative design impact cultural preservation efforts, and how they can be utilized for technologically-driven cultural preservation \cite{sabie2020, chowdhury2024, shen2025, nisi2025, bala2024}. 
Two works which more directly build technological solutions for language and culture preservation are the NLP work of \citet{lewis-yang-2012-building}, who deployed a White Hmong-English translation system which served both as an accessibility tool and a marker for cultural preservation, and the ongoing HCI work of \citet{ariyasinghe2025}, who are developing a VR experience to counteract migrant loneliness and isolation.

Our research builds upon these previous works and expands upon the use of technology for language and cultural preservation efforts through the development of a language learning game and by utilizing storytelling to create more culturally-relevant and meaningful experiences for the participants.


\subsection{Family-Based Game Design}

% HCI and CSCW have had a wide range of impacts on game design research (e.g., \cite{}). Should I use this sentence?
Previous works in HCI and CSCW have shown the importance of board and video games as a way of familial bonding (e.g., \cite{pais2025, pais2024, wen2011}) and have explored how family relationships affect learning and creating in situations where multiple parties engage with the activity or media (e.g., \cite{yu2023, druga2022, pais2024, pais2025}), a phenomenon known as joint media experiences (JME) \cite{takeuchi}.
Importantly, families within JME contexts tend to have parents take on a mentorship role, but they can sometimes take more direct control, taking away control from the children while engaging in the activity or media \cite{druga2022, einarsson2022, yu2023}.
For example, \citet{druga2022} found that parents in jointly engaged programming activities with their children performed a wide variety of roles such as mentorship---scaffolding and guiding their children, to peer collaborators---following their children's lead.
However, while \citet{einarsson2022}'s work on how father-child pairs work together in makerspace activities corroborates \citet{druga2022}'s findings regarding parental roles in creative contexts, they also found that fathers tended to take on a more commandeering/mentor role in non-technological domains, while delineating more computer-heavy tasks to their children, potentially based on a lack of experience in the medium.
This dynamic is further seen in \citet{yu2023}, who noted that, while families had a wide range of control dynamics, parents always suggested creative ideas and "gatekept" certain creative decisions (e.g., the color of a door).

Drawing upon these previous works, our research considers these family dynamics more directly by creating a game environment where the roles of the parent and child are more explicit while promoting parent-child bonding.
In our game, the child engages with the game's interface to strengthen their comprehension of the target language, while the parent takes a mentorship role, trying to guide the child towards task completion without directly engaging with the game's interface.
We believe this will balance the roles of the parent and child, allowing the child to explore while letting the parent show their knowledge without taking over the activity \cite{einarsson2022, yu2023}.
Furthermore, we plan a second phase in the design process where parents can explicitly create game scenarios they would like to see, at which point, having more physical materials for creation might prove beneficial \cite{einarsson2022}.

\subsection {Game Design for Cultural and Language Preservation}

Game design has been a popular way of sharing and celebrating cultures and traditions both in research and industry (e.g., \cite{moore2024, shen2025, ariyasinghe2025, kalinda2025, baranoski2015, jiang2025, eriksson2024, malegiannaki2020}).
The interactive and storytelling elements of games allow the audience to connect with the settings, characters and themes in a way other mediums are unable to \cite{chen2013}.
Given this, some educational language learning games have been created which utilize the medium's interactivity and unique ability to show cultures to create more culturally-relevant learning experiences (e.g., \cite{bermudez2023, cho2021, cheng2017}).
Work such as \citet{cho2021} take this a step further by having their game mechanics focus on creating immersive comprehensible input---input that challenges the learner's language skills while not being too far beyond their current ability \cite{rodrigo2004, alatis1992}.

However, culturally-relevant language learning games are not easy to develop and there needs to exist a balance between game play and education, especially when focused on comprehensible input.
Returning to the work of \citet{cho2021}, they find that their immersive, untranslated game produced similar learning outcomes to both a translated version and animation-only (non-interactive) version.
They speculate that the cognitive load new game mechanics present can sometimes detract from the language learning experience and that further research must be done on incorporating learning science principles into game design.

Thus, we take this nuanced understanding of games and language learning in mind, developing a game with simple, point-and-click mechanics.
Inspired by \citet{cho2021}, we focus on immersive comprehensible input by having only auditory cues in the target language, but expand on this by including the parent in the experience, potentially strengthening the learning experience in a way a translated game or animation could not.
Our future work will also aim to incorporate additional cultural elements and storytelling, and explore how parents help their child play the game affect their child's learning outcomes.


% HCI and CSCW have explored critical aspects of family-based and culturally-relevant game design.
% Importantly, past research in game design and the Maker Movement has shown how parents navigate making artifacts and collaborating with their children.
% \citet{druga_how_2022} explored how families jointly engage in programming activities to create games, finding that parents performed a wide variety of roles from mentors scaffolding and guiding their children, to peer collaborators following their children's lead.
% Work from \citet{einarsson2022} on how father-child pairs work together in makerspace activities corroborates \citet{druga_how_2022}'s findings, but also discusses how fathers tended to take on a more commandeering/mentor role in non-technological domains, while delineating more computer-heavy tasks to their children, potentially based on a lack of experience in the medium.
% We expand upon these works by creating a cooperative game experience for families.
% While we are not focused on developing a creative/programming space for families, we utilize their findings in our game design, creating explicit roles for the parent and child; the parents remain in a mentorship role, while the child remains in the player role due to the digital medium.



% 1. Mention HCI's role in game design
% 2. Narrow in on family-based game design
% 3. Transition into culturally-motivated game design
% 4. Language learning game design
% 5. Our work contributes to language learning game design by creating a unique experience that focuses on comprehensible auditory input within grounded real-world experiences.
% Furthermore, we plan to draw upon participants' memories and lived experiences to make future iterations of the game more reflective of their values, culture(s) and traditions. Thus, we aspire for our game to be both a language learning tool as well as a vehicle through which language and cultural promotion and preservation can occur.







% \subsection{Culture and Language Preservation with Migrant Population}

% Thing to note: migration is not always Global South to Global North; south-to-south migration is also common and remains under-explored. We are not in this space, but we need to keep this in mind, at least to know the limitations of our work.

% Broadly, answer: What has HCI done and found in this space? 
% This may need you to answer questions like: What challenges do the parents face? What roles have the researchers played?
% What gaps remain, particularly in engaging parents with children? 


% \subsection{Family-Based Game Design for Cultural and Language Preservation}

% Now, focus specifically on game design. 
% Has prior work explored games, and if so, what have they done so far? 

% Has anyone worked specifically with puzzle games? 
% If so, mention it, and detail what they found. If not, use this to justify why puzzle games are important in this space (very briefly). 



==> images/game.tex <==
\begin{figure*}
    \includegraphics[width=\linewidth]{images/Game.pdf}
    \caption{In this example, (1) the player clicks the apples, and clicks the hand to spawn an apple. (2) The player then clicks the apple to see "listen to its name", "close the menu", "eat the apple", or "pick it up". (3) The player selects "pick up" which puts the apple into the shopping cart, completing the sentence, "you put an apple in the shopping cart" This completed action is  displayed at the bottom.}
    \label{fig:game}
\end{figure*}

==> images/title.tex <==
\centering
\includegraphics[width=0.4\linewidth]{images/Title.pdf}
\captionof{figure}{Title and options menu for our game. Players can select their target language via a drop down menu in the options. All game audio will then be in the target language.}
\label{fig:title}



==> tables/participants.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}  
\centering
\begin{tabular}{@{}ll@{}}
\toprule
Particpant & Indigenous Community \\ \midrule
P6         & Bajika (Maithili)    \\
P7         & Newari*              \\
P8         & Limbu                \\
P9         & Newari               \\
P11        & Sherpa               \\
P20        & Newari               \\
P24        & Maithili             \\
P31        & Magar*               \\ \bottomrule
\end{tabular}%
\captionof{table}{Participants and their respective Indigenous communities. Those with an asterisk do not speak their community's language. Note that all participants additionally spoke English and Nepali.}
\label{tab:participants}
